AutoFS: Automated Feature Selection via Diversity-aware Interactive Reinforcement Learning

In this paper, we study the problem of balancing effectiveness and efficiency in automated feature selection. Feature selection is a fundamental intelligence for machine learning and predictive analysis. After exploring many feature selection methods, we observe a computational dilemma: 1) traditional feature selection methods (e.g., mRMR) are mostly efficient, but difficult to identify the best subset; 2) the emerging reinforced feature selection methods automatically navigate feature space to explore the best subset, but are usually inefficient. Are automation and efficiency always apart from each other? Can we bridge the gap between effectiveness and efficiency under automation? Motivated by such a computational dilemma, this study is to develop a novel feature space navigation method. To that end, we propose an Interactive Reinforced Feature Selection (IRFS) framework that guides agents by not just self-exploration experience, but also diverse external skilled trainers to accelerate learning for feature exploration. Specifically, we formulate the feature selection problem into an interactive reinforcement learning framework. In this framework, we first model two trainers skilled at different searching strategies: (1) KBest based trainer; (2) Decision Tree based trainer. We then develop two strategies: (1) to identify assertive and hesitant agents to diversify agent training, and (2) to enable the two trainers to take the teaching role in different stages to fuse the experiences of the trainers and diversify teaching process. Such a hybrid teaching strategy can help agents to learn broader knowledge, and, thereafter, be more effective. Finally, we present extensive experiments on real-world datasets to demonstrate the improved performances of our method: more efficient than existing reinforced selection and more effective than classic selection.

==> introduction.tex <==
In this paper, we aim to balance the effectiveness and efficiency in automated feature selection.
Feature selection is a fundamental intelligence for data mining and machine learning pipeline. The aim of feature selection is to select good and relevant features for downstream predictive task \cite{chandrashekar2014survey,yu2003feature}, which brings a lot of advantages. For example, the reduction of dimensionality, the improvement of prediction performance, and the comprehensibility of the result. 

Traditional feature selection can be grouped into three kinds of methods: (i) filter methods (e.g. univariate feature selection \cite{forman2003extensive}, correlation based feature selection \cite{hall1999feature}), (ii) wrapper methods (e.g. branch and bound algorithms \cite{narendra1977branch}, evolutionary algorithms \cite{kim2000feature}), and (iii) embedded methods (e.g. LASSO \cite{tibshirani1996regression}, decision tree \cite{sugumaran2007feature}). However, these methods fail to globally optimize the feature space exploration.
\begin{figure}[h]
\centering
\includegraphics[width=8.5cm,height=5cm]{pic/intro1.eps}
\caption{Comparison of IRL feature selection with reinforced feature selection. IRL feature selection integrates the advice from the teacher-like trainer.}

\label{intro1}
\vspace{-0.04cm}
\end{figure}
Recently, researchers have proposed a reinforced feature selection method \cite{fard2013using,kroon2009automatic,liu2019automating}, which formulates feature selection problem into a reinforcement learning task. 
Through this method, the process of feature selection could be automated, as reinforcement learning can automatically interact with environments and learn from action rewards for optimal decisions. However, such formulations apply stochastic exploration policy (e.g. $\epsilon-$greedy policy), making it very inefficient to find the optimal feature subset. 
%In this regard, we intend to propose a better strategy to improve reinforcement learning for feature selection.
%Previous studies of reinforced feature selection have proven to be effective in certain aspects. 
%However, these studies also have limitations. Some researchers \cite{fard2013using,kroon2009automatic} create a single agent to make decisions of the selection or deselection of all the features. Assuming there are $N$ features, the action space of the single agent is $2^N$, which makes it too difficult to find a optimal decision. As a result, other researchers \cite{liu2019automating} reformulate feature selection with multi-agent reinforcement learning. They create $N$ agents for $N$ features and each agent only needs to determine the selection of its corresponding feature. Such formulation could actually limit the action space, but it still applies stochastic exploration policy (e.g. $\epsilon-$greedy policy), making it very inefficient to find the optimal feature subset. 
%In this regard, we intend to propose a better strategy to improve reinforcement learning for feature selection.


Interactive Reinforcement Learning (IRL) is an emerging technology, which makes reinforcement learning more efficient \cite{cruz2015interactive,suay2011effect}. The intuitive idea is to include external advice in the apprenticeship of reinforcement learning to speed up the learning process. In this technology, the a concept of `teacher-like trainer' (`trainer' for short) is the source of external advice. The teacher-like trainers can be either humans or robots \cite{lin1991programming}. Also, they can be an algorithm with a priori knowledge about the desired goal 
%and can interactively encourage actions 
\cite{knox2013teaching,thomaz2006reinforcement,thomaz2005real}. Considering this, we naturally have a research question: how can we use IRL to improve the multi-agent reinforcement learning for more efficient feature selection? 
%In this paper, we call the teacher-like trainer as the trainer for simplicity.
%In traditional reinforcement learning, the action of the agent is entirely determined by its policy. Recently, researchers have proven that Interactive Reinforcement Learning (IRL) could speed up convergence of reinforcement learning. The reinforcement learning process becomes streamlined by including external advice to choose actions in the apprenticeship stages while still using agents' policies \cite{}. The external advice can come from both humans and robots \cite{} or it can be interactively given by a teacher with priori knowledge \cite{}. 

First, we intend to formulate the feature selection problem into an interactive reinforcement learning framework, where an agent is a feature selector which issues select/deselect action towards its corresponding feature. Figure \ref{intro1} shows the IRL feature selection framework.
Several challenges arise in formulating the problem.
The first challenge is to find the appropriate teacher-like trainer. In general, IRL uses human experts as trainers, which need to learn from the interactions with human experts. However, it is costly to manually teach the reinforcement learning agents, and in most cases, it is even impossible to find a human expert. Thus, can we find some trainers which do not require expert knowledge from human being, yet can still teach the reinforcement learning agent?
%However, in feature selection, human's direct recognition is largely limited by the massive data and thus of little use.
%So an obvious challenge is what teacher should we use to teach our multiple agents?
An intuitive idea is to directly use classical feature selection methods as trainers (e.g. KBest Algorithms). Thus, we propose a KBest based trainer, considering KBest feature selection \cite{forman2003extensive,yang1997comparative} could provide more insights of features by measuring feature-feature correlations, which are helpful for agents to be aware of the feature space.
%Nevertheless, there comes another problem.
However, this naive solution introduces a new problem: given a certain feature set, the KBest Algorithm always outputs the same feature subset which contains the top-$k$ features. Obviously, this trainer can only give a one-shot advice to reinforcement learning agents, while we prefer more diversified advices.
%a classical feature selection method always results in a similar optimal feature subset 
%(e.g. in KBest, the result of selecting top $k$ features and selecting top $k+1$ features only differs in one feature). 
%Taking the KBest feature selection method for example, in each iteration, given fixed input, it always outputs the same feature subset. This means when we use KBest as the trainer, it always offers the same advice, regardless of the change of the environment.
%So, the classical feature selection methods can not provide sufficient advice to reinforcement learning agents.
% line line line line
To solve this problem, we diversify advice by dynamically changing the input of the trainer. %Specifically, we dynamically select a group of features each time, which we call \textbf{participated features}, as the input to the KBest based trainer. %Furthermore, we divide the participated features into two categories: \textbf{assertive features} and \textbf{hesitant features}, whose corresponding agents are accordingly called  \textbf{assertive agents} and \textbf{hesitant agents}. Assertive features are more affirmative for agents to select, which do not need advices from trainers. Hesitant features are features that the agents are hesitant to select, which need advices from trainers by comparing them with assertive features.
%Our KBest based trainer then gives advice on the selection/deselection of hesitant features by comparing them with assertive features.
%the advised actions would be similar, which makes reinforcement learning suffer from restricted exploration.
%Actually, another challenge arises: whom should the teacher advise to? To solve this problem, we dynamically select two groups from all the agents based on their actions: namely \textbf{Assertive Agents} and \textbf{Hesitant Agents}. In each step, our KBest based teacher only advises to hesitant agents and judge whether they should change actions by comparing them to assertive agents. (need to write better than half one ?)
In this way, we formulate feature selection into an interactive reinforcement learning framework.
%interactive reinforcement learning tailored for feature selection. 

Second, after the IRL formulation, we aim to improve the efficiency of IRL. In the initial formulation, we use a KBest based trainer to guide the reinforcement learning agents. However, advices from only one trainer are not diverse enough. Thus, we try to introduce more trainers based on classical feature selection methods. Decision tree is a comparatively efficient algorithm \cite{quinlan1986induction,breiman1984classification,safavian1991survey}, which has lower computation complexity than wrapper methods (e.g.  evolutionary algorithms \cite{kim2000feature}) and has better performance than filter methods (e.g. correlation based feature selection \cite{yang1997comparative}). Also, due to its transparent nature, decision tree model allows a comprehensive analysis of features, which provides more insights for the learning process.
To take advantage of the traits of decision tree, we propose a decision tree based trainer to guide agents in IRL.
%For wrapper methods, they search on the whole feature subset space for better performance (e.g. ), which is computationally expensive and not efficient. 
%For filter methods, they are fast and efficient, and the KBest based trainer 
%we have proposed KBest based trainer, and only changing the way to calculate internal ranking scores (e.g. from univariate feature selection to correlation based feature selection) makes few differences. 
%As a result, we can only turn to wrapper methods and thus propose a Decision Tree based trainer. The feature importance of a decision tree provides a measurement of correlation among features, which could help to offer advice.
To further improve IRL algorithm, we develop a Hybrid Teaching strategy, which can make the teaching process more diversified. 
In this way, agents are guided to act more wisely after absorbing a broader range of knowledge.
%In real world, human students are usually taught by more than one teacher. Similarly, our strategy alternatively integrates experience from proposed two trainers and makes agents take advice from different trainers at different times. Therefore, agents are guided to act more wisely after absorbing a broader range of knowledge.




Third, we design an efficient reward scheme based on the history of learning process. In reinforcement learning, agents explore by taking different actions and gradually learn actions which can maximize the reward. With more and more learning, agents are more likely to choose advantageous actions. %Under the scenario of the IRL, actions are advised by teachers and tend to be more beneficial, which.
If a feature is usually chosen by an agent, it reveals this feature is important to the optimal feature subset. So, the action to select it should receive higher reward. In this regard, we make full use of historical actions and design a new reward scheme. We record the number of the times of agents selecting their corresponding features, and then use the record to weight reward assigned towards each agent. Unlike traditional sharing reward equally, this scheme personalizes the assigned reward.


In summary, in this paper, we redesign the reinforced feature selection framework based on interactive reinforcement learning. %Figure \ref{intro2} shows our contributions, 
Our contributions are as follows: (1) We formulate feature selection problem into an interactive reinforcement learning framework and we propose a KBest based trainer. (2) To offer diversified advices to agents, we propose %another trainer with a different style: 
a Decision Tree based trainer and we develop a Hybrid Teaching strategy, which integrates experience from the KBest based trainer and the Decision Tree based trainer. (3) We design an efficient reward scheme which personalizes assigned reward to multiple agents. (4) We conduct extensive experiments which demonstrates the improved performance of our methods.


%\begin{figure}[h]
%\centering
%\includegraphics[width=7.5cm,height=3.5cm]{pic/intro2.eps}
%\caption{Our main contributions}
%\label{intro2}
%\end{figure}











